ZoomLDM: Latent Diffusion Model for multi-scale image generation

Diffusion models have revolutionized image generation, yet several challenges restrict their application to large-image domains, such as digital pathology and satellite imagery. Given that it is infeasible to directly train a model on 'whole' images from domains with potential gigapixel sizes, diffusion-based generative methods have focused on synthesizing small, fixed-size patches extracted from these images. However, generating small patches has limited applicability since patch-based models fail to capture the global structures and wider context of large images, which can be crucial for synthesizing (semantically) accurate samples. To overcome this limitation, we present ZoomLDM, a diffusion model tailored for generating images across multiple scales. Central to our approach is a novel magnification-aware conditioning mechanism that utilizes self-supervised learning (SSL) embeddings and allows the diffusion model to synthesize images at different 'zoom' levels, i.e., fixed-size patches extracted from large images at varying scales. ZoomLDM synthesizes coherent histopathology images that remain contextually accurate and detailed at different zoom levels, achieving state-of-the-art image generation quality across all scales and excelling in the data-scarce setting of generating thumbnails of entire large images. The multi-scale nature of ZoomLDM unlocks additional capabilities in large image generation, enabling computationally tractable and globally coherent image synthesis up to $4096 \times 4096$ pixels and $4\times$ super-resolution. Additionally, multi-scale features extracted from ZoomLDM are highly effective in multiple instance learning experiments.

==> tables/brca_bach_sr.tex <==
\addtolength{\tabcolsep}{-0.35em}
\small
\begin{tabular}{l|c|ccccc|ccccc}
\hline
\multirow{2}{*}{Method} & \multirow{2}{*}{Conditioning} & \multicolumn{5}{c|}{TCGA BRCA} & \multicolumn{5}{c}{BACH} \\
\cline{3-12} 
 & & SSIM \textuparrow & PSNR \textuparrow & LPIPS \textdownarrow & CONCH \textuparrow & UNI  \textuparrow & SSIM \textuparrow & PSNR \textuparrow & LPIPS \textdownarrow & CONCH \textuparrow & UNI \textuparrow \\
 \hline
Bicubic & - & \textbf{0.653} & \textbf{24.370} & 0.486 & 0.871 & 0.524 & \textbf{0.895} & \textbf{34.690} & \underline{0.180} & 0.969 & \textbf{0.810} \\
CompVis \cite{rombach2022high} & LR image & 0.563 & 21.926 & \underline{0.247} & 0.946 & 0.565 & 0.723 & 27.278 & 0.206 & 0.954 & 0.576 \\
ControlNet \cite{zhang2023adding} & LR image & 0.543 & 21.980 & 0.252 & 0.874 & 0.563 & 0.780 & 27.339 & 0.276 & 0.926 & 0.721 \\
\hline
\multirow{3}{*}{ZoomLDM} & Uncond & 0.591 & 23.217 & 0.260 & 0.936 & \underline{0.680} & 0.739 & 29.822 & 0.235 & 0.965 & 0.741 \\
 & GT emb & 0.599 & 23.273 & 0.250 & \underline{0.946} & 0.672 & 0.732 & 29.236 & 0.245 & \underline{0.974} & 0.753 \\
 & Infer emb & \underline{0.609}& \underline{23.407} & \textbf{0.229} & \textbf{0.957} & \textbf{0.719} & \underline{0.779} & \underline{30.443} & \textbf{0.173} & \textbf{0.974} & \underline{0.808} \\
 \hline
\end{tabular}

==> tables/brca_large_image_fid.tex <==
\addtolength{\tabcolsep}{-0.4em}
\small
\begin{tabular}{|c||c|cc||c|cc|}
\hline
\multirow{3}{*}{Method} & \multicolumn{3}{c||}{$1024 \times 1024$} & \multicolumn{3}{c|}{$4096 \times 4096$} \\
\cline{2-7} 
& Time/ & CLIP & Crop & Time/& CLIP & Crop \\
& img & FID & FID & img & FID & FID \\
\hline
\citet{graikos2024learned} & 60 s & 7.43 & 15.51 & 4 h & 2.75 & \textbf{11.30} \\
$\infty$-Brush \cite{le2024inftybrushcontrollablelargeimage} & 30 s & 3.74 & 17.87 & 12 h & \textbf{2.63} & 14.76 l\\
ZoomLDM & 28 s & \textbf{1.23} & \textbf{14.94} & 8 m & 6.75 & 18.90 \\
\hline
\end{tabular}

==> tables/brca_mil.tex <==
\begin{tabular}{c|c|cc}
\hline
Features & Mag & Subtyping & HRD \\
\hline
Phikon \cite{filiot2023scaling} & $20\times$ & 93.81 & 76.88 \\
UNI \cite{chen2023general} & $20\times$ & 94.09 & 81.79 \\
CTransPath \cite{wang2021transpath} & $5\times$ & 93.11 & 85.37 \\
\hline
\multirow{3}{*}{ZoomLDM} & $20\times$ & 94.49 & 85.25 \\
 & $5\times$ & 94.09 & 86.26 \\
 & Multi-scale  &  \multirow{2}{*}{\textbf{94.91}} & \multirow{2}{*}{\textbf{88.03}} \\
 & ($20\times$ + $5\times$)  &  &  \\
\hline
\end{tabular}

==> tables/brca_patch_fid.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
Magnification & $20\times$ & $10\times$ & $5\times$ & $2.5\times$ & $1.25\times$ & $0.625\times$ & $0.3125\times$ & $0.15625\times$ \\
\hline
\# Training patches & 12 Mil & 3 Mil & 750k & 186k & 57k & 20k & 7k & 2.5k \\
\hline
ZoomLDM & \textbf{6.77} & \textbf{7.60} & \textbf{7.98} & \textbf{10.73} & \textbf{8.74} & \textbf{7.99} & \textbf{8.34} &\textbf{13.42} \\ 
SoTA & 6.98 \cite{graikos2024learned} & 7.64 \cite{Yellapragada_2024_WACV} & 9.74 \cite{graikos2024learned} & 20.45 & 39.72 & 58.98 & 66.28  & 106.14  \\
\hline
\hline
CDM  & 9.04 & 10.05 & 14.36 & 19.68 & 14.06 & 13.46 & 14.40 & 26.09 \\
\hline
\end{tabular}

==> tables/naip_patch_fid.tex <==
\begin{tabular}{|c|cccc|}
\hline
Resolution & 1m & 2m & 4m & 8m \\
\hline
\# Training patches & 365 k & 94 k & 25 k & 8.7 k \\
\hline
ZoomLDM & \textbf{10.93} & \textbf{7.77} & \textbf{7.34} & \textbf{8.46} \\
SoTA model & 11.5 \cite{graikos2024learned} & 23.61 & 37.52 & 65.45 \\
\hline
\end{tabular}
